Polarimetric BSSRDF Acquisition of Dynamic Faces

Acquisition and modeling of polarized light reflection and scattering help reveal the shape, structure, and physical characteristics of an object, which is increasingly important in computer graphics. However, current polarimetric acquisition systems are limited to static and opaque objects. Human faces, on the other hand, present a particularly difficult challenge, given their complex structure and reflectance properties, the strong presence of spatially-varying subsurface scattering, and their dynamic nature. We present a new polarimetric acquisition method for dynamic human faces, which focuses on capturing spatially varying appearance and precise geometry, across a wide spectrum of skin tones and facial expressions. It includes both single and heterogeneous subsurface scattering, index of refraction, and specular roughness and intensity, among other parameters, while revealing biophysically-based components such as inner- and outer-layer hemoglobin, eumelanin and pheomelanin. Our method leverages such components' unique multispectral absorption profiles to quantify their concentrations, which in turn inform our model about the complex interactions occurring within the skin layers. To our knowledge, our work is the first to simultaneously acquire polarimetric and spectral reflectance information alongside biophysically-based skin parameters and geometry of dynamic human faces. Moreover, our polarimetric skin model integrates seamlessly into various rendering pipelines.

==> backgroundc.tex <==











==> conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
We have presented a novel multispectral polarimetric 4D imaging system that includes multispectral polarization cameras, polarized light sources, and stereo imaging modules, from which we extract a video stream.
From the gathered data, we initially estimate the 3D geometry and polarimetric reflectance functions of dynamic human faces, which include the contribution of subsurface scattering and index of refraction to the global appearance.
Subsequently, we reconstruct several biophysical skin parameters from the subsurface scattering via diffusion-based multispectral optimization, which are disambiguated thanks to the accuracy of the index of refraction. 
We represent the first work to obtain spatially-varying and dynamic biophysical skin parameters (oxy-hemoglobin, deoxy-hemoglobin, eumelanin, pheomelanin, and skin base) as well as polarimetric information for dynamic human faces. 
Our skin model can be seamlessly integrated into any rendering pipeline, demonstrating its adaptability across a broad range of skin tones and facial expressions. 


==> dummy_sup.tex <==
\diego{this for now contains chunks copied and pasted from the main paper}

\mparagraph{Stokes-Mueller Formalism}
A Stokes vector represents the polarization state of a light wave and is denoted as $\mathbf{s}=[s_{0},s_{1},s_{2},s_{3}]^{\intercal}\in\mathbb{R}^{4\times1}$. 
The elements of the Stokes vector include: $s_{0}=L$, the intensity of the light; $s_{1}=L\psi\cos2\zeta\cos2\xi$, and $s_{2}=L\psi\sin2\zeta\cos2\xi$, the power of the $0\degree$ and $45\degree$ linear polarization components, respectively; and $s_{3}=L\psi\sin2\xi$, the power of the right circular polarization component. 
$\zeta$ is the polarization angle, $\xi$ is the ellipticity angle, and $\psi=\sqrt{s_{1}^{2}+s_{2}^{2}+s_{3}^{2}}/s_{0}$ is the degree of polarization (DoP), defined as the ratio of the magnitude of the polarized vector elements to the intensity of the light. The effect on the polarization of the interaction between light and any element can be represented by a Mueller matrix $\mathbf{M}\in\mathbb{R}^{4\times4}$, that transforms a Stokes vector $\mathbf{s}_{\text{in}}$ into $\mathbf{s}_{\text{out}}$ as $\mathbf{s}_{\text{out}}=\mathbf{M}\mathbf{s}_{\text{in}}$ \cite{collett2005field,wilkie_polarised_2012}. 





\mparagraph{Local coordinate system}
Polarized light has a local reference system for the angle of linear polarization. This reference has to be rotated to (and from) the coordinate system of the interaction, with is defined with respect to the plane of incidence, using a rotation Mueller matrix $\mathbf{C}(\vartheta)$~\cite{wilkie_polarised_2012}. 
Refer to Supplemental Section~\ref{supp-sec:coor-conversion} for the coordinate conversion detail. 
A common coordinate system often used for polarimetric BRDFs consists of three orthonormal vectors~\cite{hwang_sparse_2022}: the $z$-axis follows the direction of light propagation, 
the $y$-axis ($\bar{\mathbf{y}}_{i,o}$) is aligned with the camera up vector and the $x$-axis ($\bar{\mathbf{x}}_{i,o}$) is perpendicular to both. %
The plane of incidence of the specular lobe and single-scattering lobe is defined with respect to the halfway vector $\mathbf{h}$ while the diffuse lobe is defined by the surface normal $\mathbf{n}$. 




==> figure-only.tex <==










==> geometry.tex <==
\subsection{Initial Geometry}
With our multi-view system, we implement stereo matching algorithm~\cite{beeler_high-quality_2010} to estimate the depth of the face.
Although traditional stereo matching gives high quality in details, it easily suffer from the unwanted artifact in depth due to the occlusion, or discontinuity region of the face.
To handle this, we use RAFT-stereo algorithm~\cite{lipson_raft-stereo_2021} to get the good initial low resolution depth map using downsampled images.
Then, we improve the depth quality by applying stereo matching algorithm with normalized cross correlation (NCC) to generate point cloud map~\cite{beeler_high-quality_2010}.
We merge all the point cloud map in each stereo matched camera and apply Poisson surface reconstruction~\cite{kazhdan_poisson_2006} to obtain initial face geometry.
We generate uv texture map from initial geometry and all the optimized parameters are project into the uv texture map.
Note that our initial geometry then optimized further by our novel inverse-rendering.


\subsection{Tracking}
To obtain per-frame appearance parameters of dynamic face, we estimate dense 3D motion flow by tracking the mesh deformation with multi-view 2D image space tracking method~\cite{bradley_high_2010,beeler_high-quality_2011}.
We implement 3D geometry tracking by multi-view 2D image space tracking method~\cite{bradley_high_2010,beeler_high-quality_2011} to match the static scene face geometry (reference frame) across the dynamic scene frame (target frame).
Specifically, we set an anchor frame in the dynamic sequence, and estimate the 2D optical flow~\cite{teed_raft_2020,beeler_high-quality_2011} between the reference frame and the anchor frame.
To calculate the dense 2D optical flow, we use similar strategy as in Section~\ref{subsec:facegeo}. We use RAFT~\cite{teed_raft_2020} to get the low resolution 2D optical flow. Then, 2D optical flow maps are further optimized using NCC~\cite{beeler_high-quality_2011}.
Estimating the optical flow between the anchor frame and the target frame by iteratively gives correspondence between the reference frame and the any other target frame~\cite{beeler_high-quality_2011}.
Using this per-frame optical flow, we propagate the reference mesh to all other target frame in the dynamic scene progressively~\cite{bradley_high_2010}.
We perform weighted averaging to obtain final tracked mesh.


==> skin-appearance.tex <==





==> software-geometry.tex <==


\section{Dynamic Face Geometry and Tracking}
\label{sec:geometry-tracking}




\mparagraph{Face geometry}
We first acquire the base geometry of a dynamic human face from the captured stereo images and then refine geometry through inverse rendering. 
In more detail, we obtain the facial geometry from static face images captured with multi-view cameras through stereo matching~\cite{beeler_high-quality_2010, lipson_raft-stereo_2021} and Poisson surface reconstruction~\cite{kazhdan_poisson_2006}. 
With the initial geometry, we use the cylindrical texture mapping on which we define appearance and geometry parameters, including surface roughness, refractive index, and our face model parameters.
Once static capture is done, we process the dynamic captures.
First, we track corresponding points in the dynamic sequence via optical flow~\cite{teed_raft_2020,beeler_high-quality_2011}. 
With the established correspondence, we then solve for the diffuse and specular albedo of each frame in the video again by minimizing the loss between the rendering and the captured images. 



\mparagraph{Face motion tracking}
To obtain per-frame appearance parameters of dynamic face, we estimate dense 3D motion flow by tracking mesh deformation, following the multi-view 2D image-space tracking method~\cite{bradley_high_2010,beeler_high-quality_2011}. %
Specifically, we set an anchor frame in the dynamic sequence, and estimate the 2D optical flow~\cite{teed_raft_2020,beeler_high-quality_2011} between the reference frame and the anchor frame. Then, we estimate the optical flow between the anchor frame and the target frame by iteratively evaluating the correspondences between the reference frame and any other target frame~\cite{beeler_high-quality_2011}.
Using this per-frame optical flow, we propagate the reference mesh to all other target frames in the dynamic scene progressively~\cite{bradley_high_2010}.
We perform weighted averaging of per-frame tracking motions to obtain the final tracked mesh.\MIN{check what does it means with Hyunho.}



